Valuative lattices and spectra

The first part of the present article consists in a survey about the dynamical constructive method designed using dynamical theories and dynamical algebraic structures. Dynamical methods uncovers a hidden computational content for numerous abstract objects of classical mathematics, which seem a priori inaccessible constructively, e.g., the algebraic closure of a (discrete) field. When a proof in classical mathematics uses these abstract objects and results in a concrete outcome, dynamical methods generally make possible to discover an algorithm for this concrete outcome. The second part of the article applies this dynamical method to the theory of divisibility. We compare two notions of valuative spectra present in the literature and we introduce a third notion, which is implicit in an article devoted to the dynamical theory of algebraically closed discrete valued fields. The two first notions are respectively due to Huber \& Knebusch and to Coquand. We prove that the corresponding valuative lattices are essentially the same. We establish formal Valuativestellens\"atze corresponding to these theories, and we compare the various resulting notions of valuative dimensions.

==> MathMacrosSpecVal.tex <==
%!TEX encoding =  UTF-8 Unicode
%!TEX root =  mainSpv.tex

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

%: gras spéciaux

\usepackage{stixgras}
\RequirePackage{amsbsy}




%\newcommand \ix[1] {\index{#1}\textsl{#1}}

%:specialSpecVal



\newcommand{\Ndi}{\MA{\mathrm{Ndi}}}
\newcommand{\Nvr}{\MA{\mathrm{Nvr}}}
\newcommand{\Vp}{\MA{\mathrm{V}'}}
\newcommand{\Nrn}{\MA{\mathrm{Nrn}}}
\newcommand{\J}{\mathrm{J}}
\newcommand{\U}{\mathrm{Un}}
%\newcommand{\UN}{\MA{\mathrm{Un}}}

\newcommand{\rnz}{\MA{\mathrm{nz}}}

%\newcommand{\dotminus}{\mathop{\dot{-}}}
\newcommand{\sadr}{\sa{AP}}
\newcommand{\sadrp}{\sa{APp}}
\newcommand{\rdc}{rdr-clos}
\newcommand{\irdc}{ideal \rdc}
\newcommand{\ndi}{\nmid}%{{\not\vert}\;}
\newcommand{\dr}{\,\vert\hspace{-.22ex}\vert\,}
\newcommand{\drp}{\,\vert\hspace{-.22ex}\vert'\,}
\newcommand{\drd}{\;\cdot\hspace{-.7ex}\mid\,}
\newcommand \drI[1]{\,\big\vert\hspace{-.22ex}\big\vert_#1}
\newcommand \dri[1]{\,\vert\hspace{-.22ex}\vert_#1}
\newcommand \dre[1]{\,\big\vert\hspace{-.22ex}\big\vert^#1}
\newcommand \dreu[1]{\dre{{#1\uparrow\,}}}
\newcommand \dred[1]{\dre{{#1\downarrow\,}}}


\newcommand {\junk}[1]{}

%:%%%%%%%%% Cadre
\newcommand{\Cadre}[2]{%

\medskip%
\newskip\oldleftskip
\newskip\oldrightskip
\oldleftskip=\leftskip%
\oldrightskip=\rightskip%
\leftskip=-\tabcolsep%
\rightskip=-\tabcolsep%
\begin{center}\fbox{%
\begin{tabular}%
{p{#1\textwidth}}
\setlength{\parindent}{5mm}%
\vspace{-1.5mm}#2\vspace{1mm}%
\end{tabular}}\end{center}\par\medskip%
\leftskip=\oldleftskip%
\rightskip=\oldrightskip%
\setlength{\parindent}{6mm}}

%\newcommand \cm{cm}

\newcommand\boite[2]{\begin{minipage}[c]{#1cm}
     \centering {#2} \end{minipage}}
\newcommand\Boite[3]{\parbox[t][#1cm][c]{#2cm}{\boite{#2}{#3}}}


%%%%%%%%%% Encadre
\newcommand{\Encadre}[1]{\Cadre{.8}{#1}}

%%%%%%%%%% Cencadre
\newcommand{\Cencadre}[1]{\Encadre{\vspace{-3mm}
\begin{center}
#1 \end{center}\vspace{-8mm}}}

\newcommand{\cen}{\centerline}
%:  Grandcadre
\newcommand \Grandcadre[1]{%
\begin{center}
\begin{tabular}{|c|}
\hline
~\\[-3mm]
#1\\[-3mm]
~\\
\hline
\end{tabular}
\end{center}}

\newcommand\Pnv[9]{
$$\quad\quad\quad\quad
\vcenter{\xymatrix@C=1.5cm
{
#1 \ar[d]_{#2} \ar[dr]^{#3} \\
{#4} \ar@{-->}[r]_{{#5}\,!}   & {#6} \\
}}
\quad\quad
\vcenter{
\hbox{\small {#7}}
\hbox{~\\[1mm] ~}
\hbox{\small {#8}}
\hbox{~\\[-1mm] ~}
\hbox{\small {#9}}
\hbox{~\\[0mm] ~ }}
$$
}


\newcommand\dsp{\displaystyle}
\newcommand\ndsp{\textstyle}

\newcommand{\eop}{\hfill \mbox{$\Box$}}

%------- med skip et autres ---------
\newcommand \noi {\noindent}
%\renewcommand \ss {\smallskip}
\newcommand \sni {\smallskip \noi}
\newcommand \snii {\noi}
\newcommand \ms {\medskip}
\newcommand \mni {\ms\noi}
\newcommand \bs {\bigskip}
\newcommand \bni {\bs\noi}
\newcommand \hs {\qquad}
\newcommand \alb {\allowbreak}
\newcommand \ce {\centerline}

%:  Exists
%\newcommand \Exists {\rotatebox[origin=c]{180}{\tsbf{E}}\hspace{.1em}}
%\newcommand \Bot {\rotatebox[origin=c]{180}{\tsbf{T}}\hspace{.1em}}
%\newcommand \Top {{\tsbf{T}}\hspace{.1em}}

%:  leqslant
\renewcommand \le{\leqslant}
\renewcommand \leq{\leqslant}
\renewcommand \preceq{\preccurlyeq}
\renewcommand \ge{\geqslant}
\renewcommand \geq{\geqslant}
\renewcommand \succeq{\succcurlyeq}
\newcommand   \nneq {\mathrel{\#}}
\newcommand   \ineq {$_{\,\mathrel{\#}}$}

%\newcommand\tim{^\times}
\newcommand\eti{^\times}
\newcommand \epr{^\perp}
\newcommand \etl{^*}
\newcommand\sta{^\star}
\newcommand \bu {{$\bullet$}}
\newcommand \bl {^\bullet}
\newcommand{\bul}{^{\bullet}}
%\newcommand \cir {^\circ}
\newcommand \eci {^\circ}
\newcommand \ep[1]{^{(#1)}}
\newcommand \esh{^\sharp}
\newcommand \efl{^\flat}
\newcommand \eto{$^*$\xspace}
\newcommand \etoz{$^*$}
\newcommand{\edia}{^\diamond}
\newcommand{\etd}{^\triangledown}

\newcommand \ist{_\star}

\newcommand \Ast {\gA^{\!\star}}
\newcommand \Bst {\gB^{\star}}
\newcommand \iBA {_{\gB/\!\gA}}
\newcommand \iWV {_{\gW\!/\gV}}
\newcommand \Bo{\BB\mathrm{o}}
\newcommand \Ati {\gA^{\!\times}}
\newcommand \Atl {\gA^{\!*}}
\newcommand \Btl {\gB^{*}}
\newcommand \Ktl {\gK^{*}}
\newcommand{\KAt}{\gK\etl\!\sur{\Ati}}
\newcommand{\AAt}{\Atl\!\sur{\Ati}}

\newcommand \divi {\mid}

\newcommand \rdef {\mathrm{def}}

\newcommand\equidef{\buildrel{{\rdef}}\over{\;\Longleftrightarrow\;}}
\newcommand\eqdef{\buildrel{\rdef}\over {\;=\;}}
\newcommand\eqdefi{\buildrel{\rdef}\over {\;=\;}}

%------- formules a parametres --------

\newcommand \fraC[2] {{{#1}\over {#2}}}
\newcommand \formule[1]{{\left\{ {\arraycolsep2pt\begin{array}{lll} #1 \end{array}}\right.}}

\newcommand\mapright[1]{\smash{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\maprightto[1]{\smash{\mathop{\longmapsto}\limits^{#1}}}
\newcommand\mapdown[1]{\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle
#1$}}$}}
%\newcommand\Land#1{\buildrel{#1}\over \&}
\newcommand{\pref}[1]{\textup{\hbox{\normalfont(\ref{#1})}}}

\newcommand \abs[1] {\left|{#1}\right|}
%\newcommand \norm[1] {\left\parallel{#1}\right\parallel}
\newcommand \abS[1] {\big|{#1}\big|}
\newcommand \aqo[2] {#1\sur{\gen{#2}}\!}
\newcommand \Aqo[2] {#1\sur{\big\langle{#2}\big\rangle}\!}
\newcommand \Al[1] {\Vi^{\!#1}}
\newcommand \ci[1] {{{#1}^\circ}}
\newcommand \crac[2] {\cro {\frac{#1}{#2}}}
\newcommand \cro[1] {\left[#1\right]}
\newcommand \eqdf[1] {\buildrel{#1}\over =}
\newcommand \equivdf[1] {\buildrel{#1}\over \longleftrightarrow}
\newcommand \frt[1] {\!\left|_{#1}\right.\!}
\newcommand \impdef[1] {\buildrel{#1}\over \Longrightarrow}
\newcommand \norme[1]{\left\lVert #1 \right\rVert}
\newcommand \Norme[1]{\big\lVert #1 \big\rVert}
\newcommand \tra[1] {{\,^{\rm t}\!#1}}
\newcommand \gen[1] {\left\langle{#1}\right\rangle}
\newcommand \geN[1] {\big\langle{#1}\big\rangle}
\newcommand\rh[1][]{\mathrel{{\rhd}_{#1}}}
\newcommand \so[1] {\left\{ #1   \right\}}
\newcommand \sO[1]{\big\{{#1}\big\}}
%\newcommand \sotq[2]{\so{\,#1\,\vert\,#2\,}}
%\newcommand \sotQ[2]{\sO{\,#1\;\big\vert\;#2\,}}
\newcommand \sotq[2]{\so{\,#1\mathrel{;}#2\,}}
\newcommand \sotQ[2]{\sO{\,#1\mathrel{;}#2\,}}
\newcommand \sur[1] {\!\left/#1\right.}
\newcommand \und[1] {\underline{#1}}

\newcommand \Sqr {\mathrm{Sqr}}

\newcommand \idg[1] {|\,#1\,|}
\newcommand \idG[1] {\big|\,#1\,\big|}

\newcommand \norm[1] {\Vert\,#1\,\Vert}

% dimension d'une extension
\newcommand \dex[1] {[\,#1\,]}
\newcommand \deX[1] {\big[\,#1\,\big]}

% liste
\newcommand \lst[1] {[\,#1\,]}
\newcommand \lsT[1] {\big[\,#1\,\big]}


%:   fleches longues
\newcommand{\mt}{\mapsto}

\newcommand{\llongrightarrow}{\relbar\joinrel\mkern-1mu\longrightarrow}
\newcommand{\lllongrightarrow}{\relbar\joinrel\mkern-1mu\llongrightarrow}
\newcommand{\llllongrightarrow}{\relbar\joinrel\mkern-1mu\lllongrightarrow}
\newcommand\simarrow{\vers{_\sim}}
\newcommand\isosim{\buildrel{_\sim}\over \longleftrightarrow }
\newcommand\vers[1]{\buildrel{#1}\over \longrightarrow }
\newcommand\vvers[1]{\buildrel{#1}\over \llongrightarrow }
\newcommand\vvvers[1]{\buildrel{#1}\over \lllongrightarrow }
\newcommand \lora {\longrightarrow}
\newcommand \llra {\llongrightarrow}
\newcommand \lllra {\lllongrightarrow}

%:  leqslant
\renewcommand \leq{\leqslant}
\renewcommand \geq{\geqslant}

\newcommand \som {\sum\nolimits}
\newcommand \Prod {\prod\nolimits}
\newcommand \Ex {{\exists}}
\newcommand \Tt {{\forall}}
\newcommand \te {\otimes}
\newcommand \vep{{\varepsilon}}


%:  macros \`a parametres


\newcommand\lra[1]{\langle{#1}\rangle}
\newcommand\lrb[1] {\llbracket #1 \rrbracket}
\newcommand\lrbn {\lrb{1..n}}
\newcommand\lrbl {\lrb{1..\ell}}
\newcommand\lrbm {\lrb{1..m}}
\newcommand\lrbk {\lrb{1..k}}
\newcommand\lrbp {\lrb{1..p}}
\newcommand\lrbq {\lrb{1..q}}
\newcommand\lrbr {\lrb{1..r}}
\newcommand\lrbs {\lrb{1..s}}

%\newcommand \vdg {\mathrel{\vrule height6.94444pt width1pt\vrule height3.97222pt width5.11111pt depth-2.97222pt}}
% en 10pt
%\newcommand \vdg {\mathrel{\vrule height8.33333pt width1pt\vrule height4.66667pt width6.33333pt depth-3.66667pt}} % en 12pt
%\newcommand \vd {\,\,\vdg\,\,}
%\newcommand \vdi {\,\,\MA{\vdg}}

\newcommand \vda {\,\vdash\,}

\newcommand \vdw {\,\vdash_w\,}
%\newcommand \im {\rightarrow} % fleche des treillis implicatifs
\newcommand \dar[1] {\MA{\downarrow \!#1}}
\newcommand \uar[1] {\MA{\uparrow \!#1}}
\newcommand \clps[1] {{\downarrow #1\,\downarrow}}

\newcommand\tsbf[1]{\textsf{\textbf{\textup{#1}}}}
\newcommand\lab[1]{\item[\tsbf{#1}]}
\newcommand\Lab[1]{\rdb\item[\tsbf{#1}]\label{Ax#1}}
\newcommand\Tsbf[1]{\hyperref[Ax#1]{\tsbf{#1}}}

%:  mathpzc  \DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
%\newcommand\sa[1]{\hbox{\large\usefont{T1}{pzc}{m}{it}#1}\,}
%\newcommand\sab[1]{\hbox{\large\usefont{T1}{pzc}{m}{it}#1}\,\,}
\newcommand\SA[1]{\rdb\sa{#1}\label{theorie#1}}
\newcommand\Sa[1]{\hyperref[theorie#1]{\sa{#1}}}
\newcommand\sa[1]{\hbox{\usefont{T1}{pzc}{m}{it}#1}\,}
\newcommand\sab[1]{\hbox{\usefont{T1}{pzc}{m}{it}#1}\,\,}
%\newcommand\sA[1]{\hbox{\small\usefont{T1}{pzc}{m}{it}#1}\,}
\newcommand\sA[1]{\hbox{\footnotesize\usefont{T1}{pzc}{m}{it}#1}\,}
\newcommand\sAa[1]{\hbox{\footnotesize\usefont{T1}{pzc}{m}{it}#1}\,}
\newcommand\sAb[1]{\hbox{\small\usefont{T1}{pzc}{m}{it}#1}\,\,}



\newcommand \snic[1] {\smallskip \noindent \centerline{$#1$}

\smallskip }

\newcommand \snac[1]{\sni
{\small\centering$#1$\par}

\smallskip }

\newcommand \eoe {\hbox{}\nobreak\hfill
\vrule width .5em height .5em depth 0mm \par \smallskip}

%\newcommand \rF[1]{\MA{{\rm F}_{\!#1}}}
%\newcommand \rR[1]{\MA{{\rm R}_{#1}}}
%\newcommand \rRs[1]{\MA{\Rs_{#1}}}

\newcommand \bal[1] {^\rK_{#1}}
\newcommand \ul[1] {_\rK^{#1}}


\newcommand \ov[1] {\overline{#1}}


\newcommand \wh[1] {\widehat{#1} }
\newcommand \wi[1] {\widetilde{#1} }

\newcommand\dessus[2]{{\textstyle {#1} \atop \textstyle {#2}}}

\renewcommand\matrix[1]{
\begin{array}{cccccccccc} 
#1
\end{array}}

\newcommand\carray[2]{{\left[\begin{array}{#1} #2 \end{array}\right]}}
\newcommand\cmatrix[1]{\left[ \matrix{#1} \right]}
\newcommand\clmatrix[1]{{\left[\begin{array}{lllllll} #1 \end{array}\right]}}
\newcommand\dmatrix[1]{\abs{\matrix{#1}}}
\newcommand\Cmatrix[2]{\setlength{\arraycolsep}{#1}\left[\matrix{#2}\right]}
\newcommand\Dmatrix[2]{\setlength{\arraycolsep}{#1}\left|\matrix{#2}\right|}

\newcommand \bloc[4]{\left[
\begin{array}{cc}
#1 & #2   \\
#3 & #4
\end{array}
\right]}

\newcommand \cm{em}

\newcommand{\blocs}[8]{%
{\setlength{\unitlength}{.0833\textwidth}
\tabcolsep0pt\renewcommand{\arraystretch}{0}%
\begin{tabular}{|c|c|}
\hline
\parbox[t][#3\cm][c]{#1\cm}{\begin{minipage}[c]{#1\cm}
\centering#5
\end{minipage}}&
\parbox[t][#3\cm][c]{#2\cm}{\begin{minipage}[c]{#2\cm}
\centering#6
\end{minipage}}\\
\hline
\parbox[t][#4\cm][c]{#1\cm}{\begin{minipage}[c]{#1\cm}
\centering#7
\end{minipage}}&
\parbox[t][#4\cm][c]{#2\cm}{\begin{minipage}[c]{#2\cm}
\centering#8
\end{minipage}}\\
\hline
\end{tabular}
}}

\newcommand \UneCol[1]{%
\sni\mbox{\hspace{.06\textwidth}%
\parbox[t]{.94\textwidth}{#1}%
}}

\newcommand \Unecol[1]{%
\sni\mbox{\hspace{.1\textwidth}%
\parbox[t]{.9\textwidth}{#1}%
}}

\newcommand \Deuxcol[4]{%
\sni\mbox{\parbox[t]{#1\textwidth}{#3}%
\hspace{.05\textwidth}%
\parbox[t]{#2\textwidth}{#4}}}

\newcommand \DeuxCol[2]{%
\Deuxcol{.475}{.475}{#1}{#2}}

\newcommand \DeuxCols[2]{%
\sni\mbox{\hspace{.06\textwidth}%
\parbox[t]{.45\textwidth}{#1}%
\hspace{.04\textwidth}%
\parbox[t]{.45\textwidth}{#2}}}

\newcommand \DeuxRegles[2]{%
\vspace{-1.3em}\DeuxCols
{\begin{enumerate}\itemsep=0pt  #1
\end{enumerate}
}
{\begin{enumerate}\itemsep=0pt  #2
\end{enumerate}
}
\vspace{-.3em}
}

\newcommand \UneRegle[2]{%
\vspace{-1.3em}\UneCol{
\begin{enumerate}\itemsep=0pt
\lab{#1}{#2}
\end{enumerate}
}
\vspace{-.3em}
}

\newcommand \Regles[1]{%
\vspace{-1.3em}\UneCol{
\begin{enumerate}\itemsep=0pt
{#1}
\end{enumerate}
}
\vspace{-.3em}
}

\newcommand \regles[1]{%
\vspace{-1em}\Unecol{
\begin{enumerate}
{#1}
\end{enumerate}
}
\vspace{-.3em}
}

\newcommand \itbu {\item[$\bullet$]}
\newcommand \labu {\lab{$\bullet$}}

\newcommand \Deuxbu[2]{%
\vspace{-.6em}\DeuxCols
{\begin{itemize}  #1
\end{itemize}}
{\begin{itemize}  #2
\end{itemize}}}


%: revdots
\makeatletter
\def\revddots{\mathinner{\mkern1mu\raise\p@
\vbox{\kern7\p@\hbox{.}}\mkern2mu
\raise4\p@\hbox{.}\mkern2mu\raise7\p@\hbox{.}\mkern1mu}}
\makeatother

%------- lettres formatees --------
%: standards maths
\newcommand \BB{\mathbb {B}}
\newcommand \CC{\mathbb {C}}
\newcommand \FF{\mathbb {F}}
\newcommand \II{\mathbb {I}}
\newcommand \KK{\mathbb {K}}
\newcommand \MM{\mathbb {M}}
\newcommand \NN{\mathbb {N}}
\newcommand \ZZ{\mathbb {Z}}
\newcommand \OO{\mathbb {O}}
\newcommand \PP{\mathbb {P}}
\newcommand \QQ{\mathbb {Q}}
\newcommand \RR{\mathbb {R}}




% gras
\newcommand \gk {\mathbf{k}}
\newcommand \gl {\mathbf{l}}
\newcommand \gA {\mathbf{A}}
\newcommand \gB {\mathbf{B}}
\newcommand \gC {\mathbf{C}}
\newcommand \gD {\mathbf{D}}
\newcommand \gDd {\mathbf{Dd}}
\newcommand \gE {\mathbf{E}}
\newcommand \gF {\mathbf{F}}
\newcommand \gG {\mathbf{G}}
\newcommand \gI {\mathbf{I}}
\newcommand \gIo {\mathbf{Io}}
\newcommand \gK {\mathbf{K}}
\newcommand \gL {\mathbf{L}}
\newcommand \gM {\mathbf{M}}
\newcommand \gP {\mathbf{P}}
\newcommand \gQ {\mathbf{Q}}
\newcommand \gR {\mathbf{R}}
\newcommand \gRa {\mathbf{R}_\mathrm{a}}
\newcommand \gS {\mathbf{S}}
\newcommand \gT {\mathbf{T}}
\newcommand \gV {\mathbf{V}}
\newcommand \gW {\mathbf{W}}
\newcommand \gX {\mathbf{X}}
\newcommand \gz {\mathbf{z}}
\newcommand \gZ {\mathbf{Z}}

\newcommand \Red {_{\mathrm{red}}}
\newcommand \qim {_{\mathrm{min}}}
\newcommand \Ared {\gA\Red}
\newcommand \Aqim {\gA\qim}
\newcommand \Amin {\Aqim}
\newcommand \Aqi {\gA_\mathrm{qi}}



%:     SCO  (suites complementaires)
\newdimen\xyrowsp
\xyrowsp=2pt
\newcommand{\SCO}[6]{
\xymatrix @R = \xyrowsp @C =5em {
                                  &1 \ar@{-}[dl] \ar@{-}[dr] \\
#3 \ar@{-}[ddr]                   &   & #6 \ar@{-}[ddl] \\
                                  &\bullet\ar@{-}[d] \\
                                  &\bullet   \\
#2 \ar@{-}[ddr] \ar@{-}[uur]      &   & #5 \ar@{-}[ddl] \ar@{-}[uul] \\
                                  &\bullet \ar@{-}[d] \\
                                  &\bullet  \\
#1 \ar@{-}[uur]                   &   & #4 \ar@{-}[uul] \\
                                  & 0 \ar@{-}[ul] \ar@{-}[ur] \\
}
}

%:     SCo  (suites complementaires)
\newcommand{\SCo}[8]{
\xymatrix @R = #1 @C = #2{
                                  &1 \ar@{-}[dl] \ar@{-}[dr] \\
#5 \ar@{-}[ddr]                   &   & #8 \ar@{-}[ddl] \\
                                  &\bullet\ar@{-}[d] \\
                                  &\bullet   \\
#4 \ar@{-}[ddr] \ar@{-}[uur]      &   & #7 \ar@{-}[ddl] \ar@{-}[uul] \\
                                  &\bullet \ar@{-}[d] \\
                                  &\bullet  \\
#3 \ar@{-}[uur]                   &   & #6 \ar@{-}[uul] \\
                                  & 0 \ar@{-}[ul] \ar@{-}[ur] \\
}
}



%: SCOr  (suites complementaires bis)
\newcommand{\SCOr}[8]{
\xymatrix @R =1pt @C =1.2cm {
                                  &\bullet \ar@{-}[ddl] \ar@{-}[ddr] \\
                                  &#7\ar@{-}[u] \\
#3 \ar@{-}[ddr]                   &   & #6 \ar@{-}[ddl] \\
                                  &\bullet\ar@{-}[d] \\
                                  &\bullet   \\
#2 \ar@{-}[ddr] \ar@{-}[uur]      &   & #5 \ar@{-}[ddl] \ar@{-}[uul] \\
                                  &\bullet \ar@{-}[d] \\
                                  &\bullet  \\
#1 \ar@{-}[uur]                   &   & #4 \ar@{-}[uul] \\
                                  &#8\ar@{-}[d] \\
                                  &\bullet \ar@{-}[uul] \ar@{-}[uur] \\
}
}



%:  mots mathematiques rm
\newcommand \rCli {\MA{\mathrm{Cli}}}
\newcommand \Df {\MA{\mathrm{Df}}}
\newcommand \Dfr {\MA{\mathrm{Df}}^\mathrm{R}}
\newcommand \Dfmc {\MA{\mathrm{Dfmc}}}
\newcommand \rDi {\mathrm{Di}}
\newcommand \rFl {\mathrm{Fl}}
\newcommand \Mc {\mathrm{Mc}}
\newcommand \rOb {\mathrm{Ob}}
\newcommand \rmSa {\MA{\mathrm{Sa}}}
\newcommand \rmSamc {\MA{\mathrm{Samc}}}
\newcommand \DA {\rD_{\!\gA}}
\newcommand \JA {\rJ_\gA}
\newcommand \JT {\rJ_\gT}
\newcommand \oop {^{\mathrm{op}}}

\newcommand \Adj {\MA{\mathrm{Adj}}}
\newcommand \adj {\MA{\mathrm{adj}}}
\newcommand \Adu {\MA{\mathrm{Adu}}}
\newcommand \Ann {\mathrm{Ann}}
\newcommand \Atom {\mathrm{Atom}}
\newcommand \Aut {\MA{\mathrm{Aut}}}
\newcommand \BZ {\MA{\mathrm{BZ}}}
\newcommand \car {\MA{\mathrm{car}}}
\newcommand \Cl {\MA{\mathrm{Cl}}}
\newcommand \ClW {\MA{\mathrm{Cl}_{\mathrm{W}}}}
\newcommand \Coker {\MA{\mathrm{Coker}}}
\newcommand \Cont{\mathrm{Co}}
\newcommand \Dc {\MA{\mathrm{Dc}}}
\newcommand \DDiv {\MA{\mathrm{Dv}}}
\renewcommand \det {\MA{\mathrm{det}}}
\renewcommand \deg {\MA{\mathrm{deg}}}
\newcommand \Diag {\MA{\mathrm{Diag}}}
%
%\newcommand \di {\MA{\mathrm{di}}}
\newcommand \disc {\MA{\mathrm{disc}}}
\newcommand \Disc {\MA{\mathrm{Disc}}}
\newcommand \Div {\MA{\mathrm{Div}}}
\newcommand \DivA {\Div\gA }
\newcommand \DivAp {(\Div\gA)^{+} }
\newcommand \DivB {\Div\gB }
\newcommand \DivBp {(\Div\gB)^{+} }
\newcommand \DkM {\MA{\mathrm{DkM}}}
\newcommand \dv {\MA{\mathrm{div}} }
\newcommand \dvA {\dv_\gA }
\newcommand \dvB {\dv_\gB }
\newcommand \ev {{\mathrm{ev}}}
\newcommand \End {\MA{\mathrm{End}}}
\newcommand \fsac {\MA{\mathrm{fsa}}}
\newcommand \Fix {\MA{\mathrm{Fix}}}
\newcommand \Frac {\MA{\mathrm{Frac}}}
\newcommand \Gal {\MA{\mathrm{Gal}}}
\newcommand \Gfr {\MA{\mathrm{Gfr}}}
\newcommand \Gr {\MA{\mathrm{Gr}}}
\newcommand \gr {\MA{\mathrm{gr}}}
\newcommand \Gram {\MA{\mathrm{Gram}}}
\newcommand \gram {\MA{\mathrm{gram}}}
\newcommand \Grl {\MA{\mathrm{Grl}}}
\newcommand \hauteur {\mathrm{hauteur}}
\newcommand \Hom {\MA{\mathrm{Hom}}}
\newcommand \Id {\MA{\mathrm{Id}}}
\newcommand \Iv {\MA{\mathrm{Iv}}}
\newcommand \Idif {\MA{\mathrm{Idif}}}
\newcommand \Idv {\MA{\mathrm{Idv}}}
\newcommand \Ifr {\MA{\mathrm{Ifr}}}
\newcommand \Icl {\MA{\mathrm{Icl}}}
\renewcommand \Im {\MA{\mathrm{Im}}}
\newcommand \Inf {\MA{\mathrm{Inf}}}
\newcommand \Itf {\MA{\mathrm{Itf}}}
\newcommand \Ker {\MA{\mathrm{Ker}}}
%\newcommand \KR {{\MA{\mathrm{Kr}}}}
\newcommand \Lst {\MA{\mathrm{Lst}}}
\newcommand \LIN {\mathrm{Lin}}
\newcommand \Lsf {\MA{\mathrm{Lsf}}}
\newcommand \Mat {\MA{\mathrm{Mat}}}
\newcommand \Mip {\mathrm{Min}}
\newcommand \md {\mathrm{md}}
\newcommand \Mgcd {\MA{\mathrm{Mgcd}}}
%:\renewcommand \mod
\renewcommand \mod {\;\mathrm{mod}\;}
\newcommand \Mor {\MA{\mathrm{Mor}}}
\newcommand \NDc {\MA{\mathrm{NDc}}}
\newcommand \poids {\mathrm{poids}}
\newcommand \poles {\hbox {\rm p\^oles}}
\newcommand \pgcd {\MA{\mathrm{pgcd}}}
\newcommand \ppcm {\MA{\mathrm{ppcm}}}
%\newcommand \Pr {\MA{\mathrm{Pr}}}
\newcommand \Rad {\MA{\mathrm{Rad}}}
\newcommand \Reg {\MA{\mathrm{Reg}}}
%\newcommand \Rn {\MA{\mathrm{Rn}}}
\newcommand \rg{\MA{\mathrm{rg}}}
\newcommand \rgst {\mathrm{rgst}}
\newcommand \Res {\mathrm{Res}}
\newcommand \Rs {\MA{\mathrm{Rs}}}
\newcommand \rPr{\MA{\mathrm{Pr}}}
\newcommand \Rv {\mathrm{Rv}}
\newcommand \Sli {\MA{\mathrm{Sli}}}
\newcommand \Som {\MA{\mathrm{Som}}}
\newcommand \Sup {\MA{\mathrm{Sup}}}
\newcommand \Sace {\MA{\mathrm{Sace}}}
\newcommand \Smtf {\MA{\mathrm{Smtf}}}
\newcommand \Stp {\MA{\mathrm{Stp}}}
\newcommand \St {\mathrm{St}}
%\newcommand \tcl {\mathrm{tcl}}
\newcommand \Tri {\MA{\mathrm{Tri}}}
\newcommand \Tor {\MA{\mathrm{Tor}}}
\newcommand \tr {\MA{\mathrm{tr}}}
\newcommand \Tr {\MA{\mathrm{Tr}}}
\newcommand \Tsc {\MA{\mathrm{Tsch}}}
\newcommand \Um {\MA{\mathrm{Um}}}
%\newcommand \val {\MA{\mathrm{val}}}

\newcommand \SIPD {\MA{\mathrm{SIPD}}}
\newcommand \ARC {\MA{\mathrm{ARC}}}
\newcommand \AFR {\MA{\mathrm{AFR}}}
\newcommand \AFRRV {\MA{\mathrm{AFRRV}}}
\newcommand \AFRNZ {\MA{\mathrm{AFRNZ}}}
\newcommand \PPM {\MA{\mathrm{PPM}}}
\newcommand \PB {\MA{\mathrm{PB}}}

\newcommand \Suslin{{\rm Suslin}}
\newcommand{\DBxk}{{\Der \gk\gB\xi}}%
\newcommand{\DAxk}{{\Der \gk\gA\xi}}%
\newcommand{\DkXxk}{{\Der \gk\kuX\xi}}%
\newcommand \DAbul {\rD_{\!\Abul}}


%:   mots mathematiques  sf
\newcommand \sfP {\mathsf{P}}

\newcommand\MA[1]{\mathop{#1}\nolimits}

%\renewcommand \deg {\MA{\mathsf{deg}}}
\newcommand \Cdim {\MA{\mathsf{Cdim}}}
\newcommand \Divdim {\MA{\mathsf{Divdim}}}
\newcommand \Glo {\MA{\mathsf{Glo}}}
\newcommand \GK {\MA{\mathsf{GK}}}
\newcommand \GKO {\MA{\mathsf{GK}_0}}
\newcommand \HO {\MA{\mathsf{H}_0}}
\newcommand \HOp {\MA{\mathsf{H}_0^+}}
\newcommand \Hdim {\MA{\mathsf{Hdim}}}
\newcommand \HeA {{\Heit\gA}}
\newcommand \Heit {\MA{\mathsf{Heit}}}
%\newcommand \Hom {\MA{\mathsf{Hom}}}
\newcommand \Hspec {\MA{\mathsf{Hspec}}}
\newcommand \Jdim {\MA{\mathsf{Jdim}}}
\newcommand \Rdim {\MA{\mathsf{Rdim}}}
\newcommand \jdim {\MA{\mathsf{jdim}}}
\newcommand \Jspec {\MA{\mathsf{Jspec}}}
\newcommand \jspec {\MA{\mathsf{jspec}}}
\newcommand \KO {\MA{\mathsf{K}_0}}
\newcommand \KOp {\MA{\mathsf{K}_0^+}}
\newcommand \KTO {\wi{\mathsf{K}}_0}
\newcommand \Kdim {\MA{\mathsf{Kdim}}}
\newcommand \Lin {\mathsf{L}}
\newcommand \Max {\MA{\mathsf{Max}}}
\newcommand \Min {\MA{\mathsf{Min}}}
\newcommand \OQC {\MA{\mathsf{Oqc}}}
\newcommand \Pic {\MA{\mathsf{Pic}}}
\newcommand \Reel {\MA{\mathsf{Real}}}
\newcommand \Spec {\MA{\mathsf{Spec}}}
\newcommand \Speclin {\MA{\mathsf{Speclin}}}
\newcommand \Spv {\MA{\mathsf{Spv}}}
\newcommand \Spev {\MA{\mathsf{Spev}}}
\newcommand \Sper {\MA{\mathsf{Sper}}}
\newcommand \Av {\MA{\mathsf{Av}}}
\newcommand \Avd {\MA{\mathsf{Av2}}}
\newcommand \val {\MA{\mathsf{val}}}
\newcommand \vald {\MA{\mathsf{av2}}}
\newcommand \Acv {\MA{\mathsf{Acv}}}
\newcommand \Val {\MA{\mathsf{Val}}}
\newcommand \valp {\val'}
\newcommand \Valp {\Val'}
\newcommand \vals {\val\sta}
\newcommand \Vals {\Val\sta}
\newcommand \SpecA {\Spec\gA}
\newcommand \SpevA {\Spev\gA}
\newcommand \SpvA {\Spv\gA}
\newcommand \SperA {\Sper\gA}
\newcommand \SpecT {\Spec\gT}
\newcommand \Zar {\MA{\mathsf{Zar}}}
\newcommand \ZF {\MA{\mathsf{ZF}}}
\newcommand \AvA {{\Av\gA}}
\newcommand \valA {{\val\gA}}
\newcommand \ValA {{\Val\gA}}
\newcommand \valpA {{\valp\gA}}
\newcommand \ValpA {{\Valp\gA}}
\newcommand \vdima {\MA{\mathsf{vdima}}}
\newcommand \Vdim {\MA{\mathsf{Vdim}}}
\newcommand \vdim {\MA{\mathsf{vdim}}}
\newcommand \dimv {\MA{\mathsf{dimv}}}
\newcommand \ZarA {{\Zar\gA}}
\newcommand \Ri {\mathsf{Ri}}
\newcommand \Riemann {\mathsf{Riemann}}



%: calligraphique
\newcommand \cA {{\cal A}}
\newcommand \cB {{\cal B}}
\newcommand \cC {{\cal C}}
\newcommand \cD {{\cal D}}
\newcommand \cI {{\cal I}}
\newcommand \cJ {{\cal J}}
\newcommand \cF {{\cal F}}
\newcommand \cH {{\cal H}}
\newcommand \cK {{\cal K}}
\newcommand \cL {{\cal L}}
\newcommand \cM {{\cal M}}
\newcommand \cN {{\cal N}}
\newcommand \cP {{\cal P}}
\newcommand \cQ {{\cal Q}}
\newcommand \cR {{\cal R}}
\newcommand \cS {{\cal S}}
\newcommand \cT {{\cal T}}
\newcommand \cV {{\cal V}}

\newcommand \ccd{\mathcal{CD}}
\newcommand \cco{\mathcal{CO}}


\newcommand \Cin{C^{\infty}}

\newcommand \SK {\cS^\rK}
\newcommand \IK {\cI^\rK}
\newcommand \JK {\cJ^\rK}
\newcommand \IH {\cI^\rH}
\newcommand \JH {\cJ^\rH}


%: roman
\newcommand \rB {\mathrm{B}}
\newcommand \rc {\mathrm{c}}
\newcommand \I {\rI}
\newcommand \rd {\mathrm{d}}
\newcommand \rv {\mathrm{v}}
\newcommand \rI {\mathrm{I}}
\newcommand \Ic {\mathrm{Ic}}
\newcommand \rC {\mathrm{C}}
\newcommand \rD {\mathrm{D}}
\newcommand \rF {\mathrm{F}}
\newcommand \rG {\mathrm{G}}
\newcommand \rH {\mathrm{H}}
\newcommand \rJ {\mathrm{J}}
\newcommand \Li {\MA{\mathrm{Li}}}
\newcommand \rK {\mathrm{K}}
\newcommand \rL {\mathrm{L}}
\newcommand \rN {\mathrm{N}}
\newcommand \rP {\mathrm{P}}
\newcommand \rO {\mathrm{O}}
\newcommand \rR {\mathrm{R}}
\newcommand \rS {\mathrm{S}}
\newcommand \rU {\mathrm{U}}
\newcommand \rV {\mathrm{V}}
\newcommand \rZ {\mathrm{Z}}


\newcommand{\Rzero}{R_{=0}}
\newcommand{\Izero}{I_{=0}}
\newcommand{\Rnz}{R_{\neq 0}}
\newcommand{\Mnz}{M_{\neq 0}}
\newcommand{\Rvr}{R_{\Vr}}
\newcommand{\Vvr}{V_{\Vr}}
\newcommand{\Irn}{I_{\Rn}}
\newcommand{\Rrn}{R_{\Rn}}
\newcommand{\Ru}{R_{\U}}
\newcommand{\Mu}{M_{\U}}

%: gothique
\newcommand\fa{\mathfrak{a}}
\newcommand\fb{\mathfrak{b}}
\newcommand\fc{\mathfrak{c}}
\newcommand\fA{\mathfrak{A}}
\newcommand\fB{\mathfrak{B}}
\newcommand\fD{\mathfrak{D}}
\newcommand\fI{\mathfrak{i}}
\newcommand\fII{\mathfrak{I}}
\newcommand\fj{\mathfrak{j}}
\newcommand\fJ{\mathfrak{J}}
\newcommand\fF{\mathfrak{F}}
\newcommand\ff{\mathfrak{f}}
\newcommand\ffg{\mathfrak{g}}
\newcommand\fG{\mathfrak{G}}
\newcommand\fh{\mathfrak{h}}
\newcommand\fl{\mathfrak{l}}
\newcommand\fm{\mathfrak{m}}
\newcommand\fM{\mathfrak{M}}
\newcommand\fO{\mathfrak{O}}
\newcommand\fp{\mathfrak{p}}
\newcommand\fP{\mathfrak{P}}
\newcommand\fq{\mathfrak{q}}
\newcommand\fQ{\mathfrak{Q}}
\newcommand\fU{\mathfrak{U}}
\newcommand\fV{\mathfrak{V}}
\newcommand\fv{\mathfrak{v}}
\newcommand\fx{\mathfrak{x}}
\newcommand\fy{\mathfrak{y}}
\newcommand\fSpec{\mathfrak{Spec}}
\newcommand\fRie{\mathfrak{Riemann}}

\newcommand{\fDA}{\fD_\gA}
\newcommand{\fVA}{\fV_\gA}
\newcommand{\fUA}{\fU_\gA}
\newcommand{\fDB}{\fD_\gB}
\newcommand{\fVB}{\fV_\gB}
\newcommand{\fUB}{\fU_\gB}
\newcommand{\fDT}{\fD_\gT}
\newcommand{\fVT}{\fV_\gT}
\newcommand{\fUT}{\fU_\gT}

%:  mathscr  \usepackage{mathrsfs}
\newcommand \scC{\mathscr{C}}
\newcommand \scF{\mathscr{F}}
\newcommand \scG{\mathscr{G}}
\newcommand \scL{\mathscr{L}}
\newcommand \scO{\mathscr{O}}
\newcommand \scR{\mathscr{R}}
\newcommand \scU{\mathscr{U}}
\newcommand \scV{\mathscr{V}}

%: textit


%:  gras math avec \bm
\newcommand{\bma}{\bm{a}}
\newcommand{\bmb}{\bm{b}}
\newcommand{\bmc}{\bm{c}}
\newcommand{\bmd}{\bm{d}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bmu}{\bm{u}}
\newcommand{\bmv}{\bm{v}}
\newcommand{\bmw}{\bm{w}}
\newcommand{\bmy}{\bm{y}}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmz}{\bm{z}}

\newcommand \LLPO {\tsbf{LLPO}}
\newcommand \LPO  {\tsbf{LPO}}

%: penché gras
\newcommand \tslb[1]{\textbf{\textsl{#1}}}
\newcommand \slbAc {\tslb{Ac}}
\newcommand \slbAfr {\tslb{Afr}}
\newcommand \slbAo {\tslb{Ao}}
\newcommand \slbArc {\tslb{Arc}}
\newcommand \slbAzdr {\tslb{Azdr}}
\newcommand \slbAzdrz {\tslb{Azdr0}}
\newcommand \slbC{\tslb{C}}
\newcommand \slbD{\tslb{D}}
\newcommand \slbI{\tslb{I}}
\newcommand \slbL{\tslb{L}}
\newcommand \slbEAn {\tslb{EsAn}}
\newcommand \slbEs {\tslb{Es}}
\newcommand \slbFn {\tslb{Fn}}
\newcommand \slbHom {\tslb{Hom}}
\newcommand \slbMor {\tslb{Mor}}
\newcommand \slbSa {\tslb{Sa}}
\newcommand \slbSad {\tslb{Sad}}
\newcommand \Sad {\slbSad}
\newcommand \slbSet {\tslb{Set}}
\newcommand \Set {\slbSet}
\newcommand \slbTnat {\tslb{Tnat}}
\newcommand \slbTr {\tslb{Tr}}
\newcommand \slbTop {\tslb{Top}}
\newcommand \slbFa {\tslb{Fa}}
\newcommand \slbP {\tslb{P}}
\newcommand \slbPfa {\tslb{Pfa}}
\newcommand \slbTAn {\tslb{TrAn}}
\newcommand \slbTrdi {\tslb{Trdi}}
\newcommand \slbSch {\tslb{Sch}}


% anneaux, ideaux, ...
\newcommand \Zg {{\ZZ[G]}}

%: treillis distributifs
\newcommand \vu {\vee} % sup
\newcommand \vi {\wedge} % inf
%\newcommand \vii {\hbox{\,{\footnotesize $\bm{\wedge}$}\,}}
%\newcommand \vuu {\hbox{\,{\footnotesize $\bm{\vee}$}\,}}
\newcommand \Vu {\bigvee}
\newcommand \Vi {\bigwedge}
\newcommand \im {\rightarrow} % fleche des treillis implicatifs
\newcommand \da {\,\downarrow\!}
%\newcommand \ua {\,\uparrow\!}


\newcommand \vdu[1] {\vdash^{#1}}
\newcommand \vdb[1] {\vdash_{#1}}

\newcommand \Zero {\mathbf{0}}
\newcommand \Un {\mathbf{1}}
\newcommand \Deux {\mathbf{2}}
\newcommand \Trois {\mathbf{3}}
\newcommand \Quatre {\mathbf{4}}
\newcommand \Cinq {\mathbf{5}}


%:  soulign tout pret
\newcommand \una {{\underline{a}}}
\newcommand \ual {{\underline{\alpha}}}
\newcommand \ua  {{\underline{a}}}
\newcommand \ub  {{\underline{b}}}
\newcommand \ube {{\underline{\beta}}}
\newcommand \uc{{\underline{c}}}
\newcommand \ud  {{\underline{d}}}
\newcommand \udel{{\underline{\delta}}}
\newcommand \ue  {{\underline{e}}}
\newcommand \uf  {{\underline{f}}}
\newcommand \ug  {{\underline{g}}}
\newcommand \uh  {{\underline{h}}}
\newcommand \uga {{\underline{\gamma}}}
\newcommand \uP  {{\underline{P}}}
\newcommand \ur{{\underline{r}}}
\newcommand \ut{{\underline{t}}}
\newcommand \uu{{\underline{u}}}
\newcommand \ux {{\underline{x}}}
\newcommand \uxi {{\underline{\xi}}}
\newcommand \uX {\underline{X}}
\newcommand \uy{{\underline{y}}}
\newcommand \uY  {{\underline{Y}}}
\newcommand \uz{{\underline{z}}}
\newcommand \uze {{\underline{0}}}


\newcommand \ak {a_1,\ldots,a_k}
\newcommand \am {a_1,\ldots,a_m}
\newcommand \an {a_1,\ldots,a_n}
\newcommand \aq {a_1,\ldots,a_q}
\newcommand \aln {\alpha_1,\ldots,\alpha_n}
\newcommand \bn {b_1,\ldots,b_n}
\newcommand \bbm {b_1,\ldots,b_m}
\newcommand \ck {c_1,\ldots,c_k}
\newcommand \cq {c_1,\ldots,c_q}
\newcommand \gan {\gamma_1,\ldots,\gamma_n}
\newcommand \un {u_1,\ldots,u_n}
\newcommand \xk {x_1,\ldots,x_k}
\newcommand \Xk {X_1,\ldots,X_k}
\newcommand \xm {x_1,\ldots,x_m}
\newcommand \Xm {X_1,\ldots,X_m}
\newcommand \sn {s_1,\ldots,s_n}
\newcommand \xn {x_1,\ldots,x_n}
\newcommand \xzn {x_0,\ldots,x_n}
\newcommand \azn {a_0,\ldots,a_n}
\newcommand \bzn {b_0,\ldots,b_n}
\newcommand \yzn {y_0,\ldots,y_n}
\newcommand \zzn {z_0,\ldots,z_n}
\newcommand \uzn {u_0,\ldots,u_n}
\newcommand \xhn {x_0:\ldots:x_n}
\newcommand \Xn {X_1,\ldots,X_n}
\newcommand \xr {x_1,\ldots,x_r}
\newcommand \Xr {X_1,\ldots,X_r}
\newcommand \xin {\xi_1,\ldots,\xi_n}
\newcommand \xizn {\xi_0,\ldots,\xi_n}
\newcommand \xihn {\xi_0:\ldots:\xi_n}
\newcommand \ym {y_1,\ldots,y_m}
\newcommand \yr {y_1,\ldots,y_r}
\newcommand \Yr {Y_1,\ldots,Y_r}
\newcommand \Ym {Y_1,\ldots,Y_m}
\newcommand \Yn {Y_1,\ldots,Y_n}
\newcommand \yn {y_1,\ldots,y_n}

\newcommand \AT {\gA[T]}
\newcommand \AX {\gA[X]}
\newcommand \AuX {\gA[\uX]}
\newcommand \Aux {\gA[\ux]}
\newcommand \ArX {\gA\lra X}
\newcommand \Axn {\gA[\xn]}
\newcommand \AXn {\gA[\Xn]}

\newcommand \AXm {\gA[\Xm]}
\newcommand \KKXm {{\KK[\Xm]}}
\newcommand \KKuX {{\KK[\uX]}}

\newcommand \AY {\gA[Y]}
\newcommand \Ayn {\gA[\yn]}

\newcommand \BuX {\gB[\uX]}
\newcommand \BuY {\gB[\uY]}
\newcommand \BX {{\gB[X]}}
\newcommand \BT {{\gB[T]}}
\newcommand \BY {{\gB[Y]}}
\newcommand \Bxn {\gB[\xn]}
\newcommand \BXn {{\gB[\Xn]}}
\newcommand \BYm {\gB[\Ym]}

\newcommand \CT {{\gC[T]}}
\newcommand \CX {{\gC[X]}}
\newcommand \CXn {{\gC[\Xn]}}

\newcommand \kX {{\gk[X]}}
\newcommand \KX {\gK[X]}
\newcommand \KT {\gK[T]}
\newcommand \KuX {\gK[\uX]}
\newcommand \kuX {\gk[\uX]}
\newcommand \Kux {\gK[\ux]}
\newcommand \kux {\gk[\ux]}
\newcommand \KXk {\gK[\Xk]}
\newcommand \KXm {\gK[\Xm]}
\newcommand \KXn {\gK[\Xn]}
\newcommand \kxm {\gk[\xm]}
\newcommand \kxn {\gk[\xn]}
\newcommand \kXn {\gk[\Xn]}
\newcommand \KYm {\gK[\Ym]}
\newcommand \kXr {\gk[\Xr]}
\newcommand \KXr {\gK[\Xr]}
\newcommand \Kxr {\gK[\xr]}

\newcommand \KuY {\gK[\uY]}
\newcommand \Kuy {\gK[\uy]}
\newcommand \Kyn {\gK[\yn]}
\newcommand \Kyr {\gK[\yr]}
\newcommand \kYr {\gk[\Yr]}
\newcommand \KYr {\gK[\Yr]}
\newcommand \Kxn {\gK[\xn]}

\newcommand \LuX {\gL[\uX]}
\newcommand \lXn {\gl[\Xn]}
\newcommand \lxn {\gl[\xn]}
\newcommand \LXn {\gL[\Xn]}
\newcommand \lXr {\gl[\Xr]}
\newcommand \LXr {\gL[\Xr]}
\newcommand \lYr {\gl[\Yr]}
\newcommand \LYr {\gL[\Yr]}

\newcommand \QQXn {\QQ[\Xn]}

\newcommand \Rx {\gR[x]}
\newcommand \Rux {\gR[\ux]}
\newcommand \RuX {\gR[\uX]}
\newcommand \RXk {{\gR[\Xk]}}
\newcommand \RXm {{\gR[\Xm]}}
\newcommand \Rxm {{\gR[\xm]}}
\newcommand \RXn {{\gR[\Xn]}}
\newcommand \Rxn {{\gR[\xn]}}
\newcommand \RXzn {{\gR[\Xzn]}}
\newcommand \Rxzn {{\gR[\xzn]}}
\newcommand \RXr {\gR[\Xr]}

\newcommand \Ruy {\gR[\uy]}
\newcommand \Ryn {{\gR[\yn]}}
\newcommand \RRX {\RR[X]}
\newcommand \RRXn {\RR[\Xn]}
\newcommand \RRxn {\RR[\xn]}
\newcommand \RYr {\gR[\Yr]}
\newcommand \RRuX {\RR[\uX]}
\newcommand \RRux {\RR[\ux]}

\newcommand \CCX {\CC[X]}

\newcommand \ZZXn {\ZZ[\Xn]}
\newcommand \ZG {\ZZ[G]}

\newcommand \RRXk {{\RR[\Xk]}}
\newcommand \RRxk {{\RR[\xk]}}
\newcommand \RRXm {{\RR[\Xm]}}
\newcommand \RRxm {{\RR[\xm]}}
%\newcommand \RRXn {{\RR[\Xn]}}


\newcommand \lfs {f_1,\ldots,f_s}


%:  Foncteurs grasmanniennes, GLn,SLn ...
\newcommand \Gn  {\gG_n}
\newcommand \Gnk {\gG^n_{k}}
\newcommand \Gnr {\gG^n_{r}}
\newcommand \cGn {\cG_n}
\newcommand \cGnk{\cG_{n,k}}
\newcommand \GGn {\GG^n}
\newcommand \GGnk{\GGn_{k}} % Grasmannienne ``projective'' usuelle
\newcommand \GGnr{\GGn_{r}}
\newcommand \GA  {\mathbb{GA}}
\newcommand \GAn {\GA^n}  % Grasmannienne ``affine'': matrices de proj
\newcommand \GAq {\GA^q}
\newcommand \GAnk{\GAn_{k}}
\newcommand \GAnr{\GAn_{r}}
\newcommand \GL {\mathbb{GL}}
\newcommand \GLn {{\GL_n}}
\newcommand \SL {\mathbb{SL}}
\newcommand \SLn {{\SL_n}}
\newcommand \EE {\mathbb{E}}
\newcommand \En {\EE_n}
\newcommand \Pn {\PP^n}
\newcommand \An {\AA^n}
\newcommand \Sl {\mathbf{SL}}
\newcommand \Sln {{\Sl_n}}


\newcommand \Mm {\MM_{m}}
\newcommand \Mn {\MM_{n}}
\newcommand \Mk {\MM_{k}}
\newcommand \Mq {\MM_{q}}
\newcommand \Mr {\MM_{r}}
\newcommand \MMn {\MM_{n}}


\newcommand \Pf {{{\cal P}_{\mathrm{f}}}}
\newcommand \Pfe {{\rm P}_{{\rm fe}}}



%: hsu
\newcommand\hsz{\\ }
\newcommand\hsu{\\ \hspace*{4mm}}
\newcommand\hsd{\\ \hspace*{8mm}}
\newcommand\hst{\\ \hspace*{1,2cm}}
\newcommand\hsq{\\ \hspace*{1,6cm}}
\newcommand\hsc{\\ \hspace*{2cm}}
\newcommand\hsix{\\ \hspace*{2,4cm}}
\newcommand\hsept{\\ \hspace*{2,8cm}}







%

